Prophets, Secretaries, and Maximizing the Probability of Choosing the Best

Suppose a customer is faced with a sequence of fluctuating prices, such as for airfare or a product sold by a large online retailer. Given distributional information about what price they might face each day, how should they choose when to purchase in order to maximize the likelihood of getting the best price in retrospect? This is related to the classical secretary problem, but with values drawn from known distributions. In their pioneering work, Gilbert and Mosteller [\textit{J. Amer. Statist. Assoc. 1966}] showed that when the values are drawn i.i.d., there is a thresholding algorithm that selects the best value with probability approximately $0.5801$. However, the more general problem with non-identical distributions has remained unsolved. In this paper we provide an algorithm for the case of non-identical distributions that selects the maximum element with probability $1/e$, and we show that this is tight. We further show that if the observations arrive in a random order, this barrier of $1/e$ can be broken using a static threshold algorithm, and we show that our success probability is the best possible for any single-threshold algorithm under random observation order. Moreover, we prove that one can achieve a strictly better success probability using more general multi-threshold algorithms, unlike the non-random-order case. Along the way, we show that the best achievable success probability for the random-order case matches that of the i.i.d.\ case, which is approximately $0.5801$, under a "no-superstars" condition that no single distribution is very likely ex ante to generate the maximum value. We also extend our results to the problem of selecting one of the $k$ best values.

==> PS.tex <==
\section{What we know on Prophet Secretary}
If for some constant $\eps$ the contribution of one distribution to the optimum is $\eps \OPT$ then there is a single threshold algorithm that gets $1-1/e +\eps'$ approximation, where $\eps'$ is a constant depends on (and much smaller than) $\eps$.

When the contribution of each distribution tends to $0$, an algorithm that uses threshold $\tau_1 = F^{-1}(\theta_1)$ on the first $n/2$ items and $\tau_2 = F^{-1}(\theta_2)$ on the last $n/2$ items gets
$$ (1-\theta_1^{1/2})\Big(\tau_1+\frac{-1}{\ln \theta_1}\ex{(\OPT-\tau_1)^+}\Big)  + \theta_1 (1-\theta_2^{1/2})\Big(\tau_2+\frac{-1}{\ln \theta_2}\ex{(\OPT-\tau_2)^+}\Big)  $$.
%
If we set $\tau_1=\tau_2=F^{-1}(1/e)$ the above equation gives us $(1-1/e)(\tau+\ex{(\OPT-\tau)^+}) \leq (1-1/e)\OPT$.

The above inequality is not tight unless $\ex{\min(\tau,\OPT)}\simeq \tau$. Otherwise, if $\tau \geq \eps \OPT$ the current threshold gives a $1-1/e+\eps'$ approximate solution. If $\tau > \eps \OPT$, $\tau'=F^{-1}(1/e-\epsilon)$ gives us a $1-1/e+\eps'$ approximate solution.

Followings are a couple of good example. They are both $n$ iid distributions. Always  $F^{-1}(1/e-\epsilon)=F^{-1}(1/e+\epsilon)$
\begin{itemize}
	\item $1$ with probability $1-1/n^2$ and $n^3$ otherwise (we should not bring the threshold bellow $F^{-1}(1/e)$).
	\item $e-2$ with probability $1-1/n^2$ and $n+R$ otherwise (for $R=0$, $F^{-1}(1/e)$ is tight for positive $R$ we prefer to bring the single threshold up for negative $R$ we prefer to bring the single threshold down.)
\end{itemize}




==> reduction.tex <==
\section{Reduction to IID setting}

In this section we show that the worst-case instances for best-or-nothing prophet secretary are, in fact, iid.  We'll actually show something stronger: for any sequence of thresholds $\Tau = \langle \tau_1,\ldots, \tau_n \rangle$, there is a worst-case instance for the threshold algorithm $\Tau$ that is iid.  (We will use $\Tau$ to refer to both a sequence of thresholds and to the corresponding threshold algorithm.)

\begin{claim}
Fix any threshold sequence $\Tau$, and any set of distributions $D_1, \dotsc, D_n$ for which $\Tau$ selects the maximum element with probability $\alpha$.  Then on the iid instance with distribution $D$ such that $D(x) = \left( \prod_i D_i(x) \right)^{1/n}$ for all $x$, $\Tau$ selects the maximum element with probability at most $\alpha$.
\end{claim}

We'll prove the claim in three steps.  First, we'll couple the outcome of the prophet secretary process to a simpler, more discrete process.  We'll then argue that the failure probability in this simpler process is monotone with respect to a certain measure on realized values.  Finally, we'll show that the proposed iid distribution maximizes this measure.

\subsection{An Equivalent Process}

Fix $\Tau = \langle \tau_1,\ldots, \tau_n \rangle$, with $\tau_1 \geq \dotsc \geq \tau_n$.  Write $\tau_0 = \infty$ and $\tau_{n+1} = 0$ for notational convenience.  Write $I_j$ for the interval $[\tau_{n+1-j}, \tau_{n-j})$ for $0 \leq j \leq n$.  That is, $I_0$ spans the lowest values, and $I_n$ spans the highest values.  For each distribution $D_i$, define a discrete distribution $F_i$ over $\{0, 1, \dotsc, n\}$, with PDF $f_i$, such that $f_i(j) = Pr_{x \sim D_i}[ x \in I_j ]$.  We'll write $F_i$ both for the CDF of this distribution, and for the distribution itself.

There is a natural coupling between $F_i$ and $D_i$, in which $x_i \sim D_i$ is coupled with value $k_i$ if and only if $x_i \in I_{k_i}$.  We can interpret this coupling as follows: $k_i \sim F_i$ indicates that there are exactly $k_i$ steps of the prophet secretary process in which the realized value $x_i \sim D_i$ is higher than the corresponding threshold in that step.  E.g., if $k_i = 3$, then $x_i$ lies above the final three thresholds, corresponding to the final 3 steps, but lies below all other thresholds.

Consider now the following process.  We draw $k_i \sim F_i$ for each $i$.  We then draw a random permutation $\langle \pi_1, \dotsc, p_n \rangle$, where $\pi_k$ is the item shown in step $n-k+1$.  (I.e., $\pi_1$ is the item shown last.)  We'll also write $\sigma_i$ for the value $j$ such that $\pi_j = i$.  Choose $i^*$ such that $k_{i^*}$ is maximized, breaking ties arbitrarily.  We will say that this instance is \emph{successful} if the following are true:
\begin{enumerate}
\item $\sigma_{i^*} \leq k_{i^*}$
\item for each $j \neq i^*$, either $\sigma_j > k_{i^*}$ or $\sigma_j < \sigma_{i^*}$.
\end{enumerate}
We claim that a realized instance of best-or-nothing prophet secretary picks the maximum value if and only if its coupled instance of the process above is successful.  Indeed, $i^*$ is the index of the item with highest realized value, noting that we will break ties in the specification of $i^*$ to maintain this coupling.  The condition $\sigma_{i^*} \leq k_{i^*}$ corresponds to value $x_{i^*}$ lying above the threshold on the step in which it appears.  The condition that $\sigma_j > k_{i^*}$ or $\sigma_j < \sigma_{i^*}$ is equivalent to enforcing that there is no other value $x_j$ that appears before $x_{i^*}$ in the permutation that also lies above its corresponding threshold.  These are precisely the conditions needed for $i^*$ to be selected by the algorithm.

Define discrete distribution $F$ such that, for each $k$, $F(k) = \left( \prod_i F_i(k) \right)^{1/n}$.  To prove our reduction, it suffices to show that the probability of success under the iid problem with distribution $F$ is at most the probability of success under distributions $F_1, \dotsc, F_n$.

\subsection{Characterizing the Probability of Success}

(Sketch -- this needs more formalization.)

Suppose that $\sigma_{i^*} = \theta$.  In order for the instance to be successful, there must be at least one $j$ such that $k_j \geq \theta$ (namely, $j = i^*$).  For each $k$, write $\ell_k$ for the cardinality of the set $L_k = \{ j \colon k_j \geq k\}$.

Suppose that $\ell_{\theta+1} \geq 1$.  Then the probability that item $\pi_{\theta + 1}$ violates the second condition of success is $\frac{\ell_{\theta+1} - 1}{n-1}$, the probability that $\pi_{\theta+1}$ is one of the items in set $L_{\theta+1}$, after excluding $i^*$.  

If we condition on the event above not occuring, and we suppose that $\ell_{\theta+2} \geq 1$, then the probability that item $\pi_{\theta + 2}$ violates the second condition of success is $\frac{\ell_{\theta+2}-1}{n-2}$.  Again, this is the probability that $\pi_{\theta+2}$ is one of the items in set $L_{\theta+2}$, after excluding $i^*$ and $\pi_{\theta+1}$.  Note that due to our conditioning, we have that $\pi_{\theta+1} \not\in L_{\theta+1}$, and hence $\pi_{\theta+1} \not\in L_{\theta+2}$ as well.

Repeating this argument, the probability that success is violated by item $\pi_k$ with $k > \theta$, conditional on it not being violated by prior items and conditional on there being at least one item with $k_j \geq k$, is $\frac{\ell_{k}-1}{n-k}$.  Thus, all else being equal, the probability of failure increases as the expected number of items for which $k_j \geq k$ (conditional on there being at least one) increases.

\subsection{An Extremal Lemma}

\begin{lemma}
Fix $p_1, \dotsc, p_n \in [0,1]$, and set $p = \left(\prod_i p_i \right)^{1/n}$.  Let $X$ be a R.V. denoting the number of successes of bernoulli trials with probabilities $p_1, \dotsc, p_n$, and $Y$ denote the number of successes of $n$ bernoulli trials each with probability $p$.  Then $E[X] \geq E[Y]$.
\end{lemma}
\begin{proof}
Take $n=2$ and suppose $p_1 < p_2$, say with $p_2 = \beta \cdot p_1$ where $\beta > 1$.  Write $p'_1 = \alpha \cdot p_1$ and $p'_2 = p_2 / \alpha$, where $1 < \alpha < \beta$.  Then we will show that $E[X] \geq E[Z]$, where $Z$ is the number of successes of bernoulli trials with probabilities $p'_1$ and $p'_2$.  This will suffice to prove the claim, since one can move from $p_1, \dotsc, p_n$ to $p, \dotsc, p$ using a finite number of alterations of a single pair of coordinates, increasing the number of coordinates equal to $p$ at each step.

We'll now prove the claim.  The probability that $X = 2$ is equal to the probability that $Z = 2$, by construction.  So it remains to show that $Pr[X = 0] \leq Pr[Z = 0]$.  Well, we have
\begin{align*}
Pr[Z = 0] & = (1 - p'_1)(1 - p'_2) \\
& = (1 - \alpha \cdot p_1)(1 - p_2 / \alpha ) \\
& = 1 - \alpha \cdot p_1 - \beta \cdot p_1 / \alpha + p_1 \cdot p_2 \\
& \geq 1 - p_1 - \beta \cdot p_1 + p_1 \cdot p_2 \\
& = Pr[X = 0]
\end{align*}
where the inequality follows because, for $\alpha > 1$, $\alpha + \beta/\alpha \leq 1 + \beta$ if and only if $\alpha \leq \beta$.
\end{proof}

The lemma implies that, for any given $k$, if we keep constant the probability that there is at least one item with $k_j \geq k$ (i.e., by keeping constant the product $\prod_i F_i(k)$), then the expected number of items for which $k_j \geq k$ is maximized by setting $F_i(k) = F(k)$ for all $i$.  Thus, taking $F_i = F$ for all $i$ will maximize the probability of failure at each step independently, and must therefore also maximize the probability of failure overall.

